LLM4GEN: Leveraging Semantic Representation of LLMs for Text-to-Image Generation

Diffusion models have exhibited substantial success in text-to-image generation. However, they often encounter challenges when dealing with complex and dense prompts involving multiple objects, attribute binding, and long descriptions. In this paper, we propose a novel framework called \textbf{LLM4GEN}, which enhances the semantic understanding of text-to-image diffusion models by leveraging the representation of Large Language Models (LLMs). It can be seamlessly incorporated into various diffusion models as a plug-and-play component. A specially designed Cross-Adapter Module (CAM) integrates the original text features of text-to-image models with LLM features, thereby enhancing text-to-image generation. Additionally, to facilitate and correct entity-attribute relationships in text prompts, we develop an entity-guided regularization loss to further improve generation performance. We also introduce DensePrompts, which contains $7,000$ dense prompts to provide a comprehensive evaluation for the text-to-image generation task. Experiments indicate that LLM4GEN significantly improves the semantic alignment of SD1.5 and SDXL, demonstrating increases of 9.69\% and 12.90\% in color on T2I-CompBench, respectively. Moreover, it surpasses existing models in terms of sample quality, image-text alignment, and human evaluation.

==> sections/checklist.tex <==
\subsection{Paper Checklist}

\noindent This paper
\begin{enumerate}
    \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced. \textbf{Yes.}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results.\textbf{ Yes.}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. \textbf{Yes.}
\end{enumerate}
\noindent Does this paper make theoretical contributions? \textbf{No.}

\noindent Does this paper rely on one or more datasets? \textbf{Yes.}

\noindent If yes, please complete the list below.
\begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets. \textbf{Yes.}
    \item All novel datasets introduced in this paper are included in a data appendix. \textbf{NA.}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{NA.}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{Yes.}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{Yes.}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textbf{NA}
    
\end{enumerate}

\noindent Does this paper include computational experiments? \textbf{Yes.}

\noindent If yes, please complete the list below.
\begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix. \textbf{Yes.}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{Yes.}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{Yes.}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textbf{Yes.}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{Yes.}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{Yes.}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{Yes.}
    \item This paper states the number of algorithm runs used to compute each reported result. \textbf{Yes.}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{Partial.}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{Yes.}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{Partial.}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{Partial.}
\end{enumerate}
